DOR3D-Net: Dense Ordinal Regression Network for 3D Hand Pose Estimation

Depth-based 3D hand pose estimation is an important but challenging research task in human-machine interaction community. Recently, dense regression methods have attracted increasing attention in 3D hand pose estimation task, which provide a low computational burden and high accuracy regression way by densely regressing hand joint offset maps. However, large-scale regression offset values are often affected by noise and outliers, leading to a significant drop in accuracy. To tackle this, we re-formulate 3D hand pose estimation as a dense ordinal regression problem and propose a novel Dense Ordinal Regression 3D Pose Network (DOR3D-Net). Specifically, we first decompose offset value regression into sub-tasks of binary classifications with ordinal constraints. Then, each binary classifier can predict the probability of a binary spatial relationship relative to joint, which is easier to train and yield much lower level of noise. The estimated hand joint positions are inferred by aggregating the ordinal regression results at local positions with a weighted sum. Furthermore, both joint regression loss and ordinal regression loss are used to train our DOR3D-Net in an end-to-end manner. Extensive experiments on public datasets (ICVL, MSRA, NYU and HANDS2017) show that our design provides significant improvements over SOTA methods.

==> supply.tex <==
we analyze statistics of the hand $z$ coordinate distribution in public datasets (Fig. \ref{fig_norm}) and notice that it is close to normal distribution (ND).

\noindent
\begin{figure}[t]
\centering
\includegraphics[width=1.0\columnwidth]{figure/figure_norm} 
\caption{The depth distribution of joints on HANDS2017, MSRA, NYU, and ICVL datasets, which are close to normal distribution.
}
\label{fig_norm}
\end{figure}

Fig. \ref{fig2} illustrates the pipeline of the Swin Transformer-based feature extractor used in our work.

\begin{figure*}[t]
\centering
\includegraphics[width=0.8\textwidth]{figure/figure2} 
\caption{The pipeline of our transformer-based feature extractor. 
It contains patch partition and four Swin Transformer stages. 
Patch partition splits the image into multiple $4\times4$ patches and each patch is considered as a token. 
Then tokens pass through each stage to learn long-range feature interactions through Swin Transformer blocks. 
The final two feature maps from the last stage are sent into the 
ordinal regression module for 3D hand pose prediction.}
\label{fig2}
\end{figure*}




The 3D per-joint mean error and the percentages of success frames over different error thresholds are shown in Fig. \ref{figure6}.


\begin{figure*}[t]
\centering
\vspace{-0.35cm} 
\subfigtopskip=1pt 
\subfigbottomskip=0pt 
\centering
\subfigure[3D per-joint mean error on MSRA]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.30in]{figure/msra_error_1}
\end{minipage}
}

\centering
\subfigure[3D per-joint mean error on ICVL]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.30in]{figure/icvl_error_1}
\end{minipage}
}

\centering
\subfigure[3D per-joint mean error on NYU]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.30in]{figure/nyu_error_1}
\end{minipage}
}

\subfigbottomskip=0pt 
\centering
\subfigure[Proportion of good frames on MSRA]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.25in]{figure/msra_error_2}
\end{minipage}
}

\centering
\subfigure[Proportion of good frames on ICVL]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.30in]{figure/icvl_error_2}
%\caption{fig2}
\end{minipage}%
}

\centering
\subfigure[Proportion of good frames on NYU]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.30in]{figure/nyu_error_2}
\end{minipage}
}

\caption{
Comparison with the state-of-the-art methods on MSRA, ICVL, and NYU dataset.
Top: The per-joint mean error for all the test examples.
Bottom: Percentage of frames in the testing examples under
different error thresholds.
}
\label{figure6}
\end{figure*}



In order to intuitively verify our method, we make some changes to the full model: (1) Replace the transformer with Resnet50; 
(2) Replace the ordinal classifier with offset-based regression. Fig. \ref{fig7} visualizes and compares the hand pose estimation results. In each image, the color in yellow, red, green, blue, and pink represents five fingers respectively. The bright colors denote estimated joints and the dark are the ground truth. 
It can be seen that our full model has better performance on edge blur, background noise and occlusion cases, while the other two variants predict worse joints' position which may suffer from outliers and low-level feature representation.


\noindent
\begin{figure}[t]
\centering
\includegraphics[width=1.0\columnwidth]{figure/figure7}
\caption{Qualitative comparison results on HANDS2017.
Bright colors: predicted joints.
Dark colors: ground truth.
Top: without transformer.
Middle: without ordinal regression.
Bottom: ours full model.}

\label{fig7}
\end{figure}
